Designing novel protein structures using sequence generator and AlphaFold2

Protein structures and functions are determined by a contiguous arrangement of amino acid sequences. Designing novel protein sequences and structures with desired geometry and functions is a complex task with large state spaces. Here we develop a novel protein design pipeline consisting of two deep learning algorithms, ProteinSolver and AlphaFold2. ProteinSolver is a deep graph neural network that generates amino acid sequences such that the forces between interacting amino acids are favorable and compatible with the fold while AlphaFold2 is a deep learning algorithm that predicts the protein structures from protein sequences. We present forty de novo designed binding sites of the PTP1B and P53 proteins with high precision, out of which thirty proteins are novel. Using ProteinSolver and AlphaFold2 in conjunction, we can trim the exploration of the large protein conformation space, thus expanding the ability to find novel and diverse de novo protein designs.

==> reference.tex <==
\iffalse


\begin{figure}[ht!] 
 \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/2-148-mp-30357.png}
        \caption{SrTiO3(Target)}
        \vspace{-3pt}
        \label{fig:La3Al1N1}
    \end{subfigure}
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/2-148-mp-30357.png}
        \caption{Ni3S4(Target)}
        \vspace{-3pt}
        \label{fig:La3Al1N1}
    \end{subfigure}    
    \begin{subfigure}[t]{0.33\textwidth}
        \includegraphics[width=\textwidth]{figures/2-148-mp-30357.png}
        \caption{NiS2(Target)}
        \vspace{-3pt}
        \label{fig:La3Al1N1}
    \end{subfigure}    
  \caption{Exceptional structures for our building block extraction algorithm. (a)xxxxx.(b) .... (c)...}
  \label{fig:predictedstructures}
\end{figure}


Our building block detection algorithm is based on the logic that if the distance between two nearby is equal to the sum of their radii, then the two atoms are bonded. Instead of comparing every atom to every other atom within a given structure, we used the CrystalNN algorithm to determine a starting set of potential neighbors for each atom. CrystalNN did not detect building blocks in this data set well enough on its own to be used without modification. 

\textbf{todo: define ionic vs covalent and why their bond lengths are different}

Atomic radius alone is not an accurate standard for all bonds since bond type can affect the distance between two atoms.  Since our algorithm compares distance and the sum of the radii between two nearby atoms, it was important to have accurate radii for every possible combination of atoms. Therefore, we had to determine if each bond was ionic or covalent. Ionic bonds form when the difference in electronegativity between two sites is greater than 1.7. If the electronegativity difference was found to be less than 1.7, we used the covalent radius provided by pymatgen, otherwise we tried to find the oxidation state of the elements being compared. \textbf{EXPLAIN WHY FINDING OXI STATE WAS IMPORTANT} In some cases, pymatgen's oxidation state prediction tool would fail. Most of these cases were similar to \textbf{Figure "D:\sorted-symmetrized-cifs\QuickCheck\NoBonds\Incorrect\2-148-mp-30357.cif" }, so it did not matter that it was unable to determine the correct radius to use because there were no bonds to be found. However, some cases where the oxidation state prediction tool failed had valid building blocks, so the atomic radius was used as a placeholder.

We also limited the types of bonds that could be added to a building block. We only allowed the following kinds of bonds, where the first type of atom listed is the center atom and the second is the satellite atom: metal to metal, metal to metalloid, metalloid to metalloid, metalloid to nonmetal, and nonmetal to nonmetal. If the center of a building block was a nonmetal, it did not make sense to allow it to 


\subsection{Composition based structural building block prediction}


Magpie descriptors are a set of features that contain a variety of chemical and physical properties to transform raw materials data into a form compatible with machine learning. There are four kinds of categories in Magpie descriptors, including stoichiometric features, elemental property statistics, electronic structure features, and ionic compound features. All those features can be generated by the given stoichiometry (formula) of a material. In our experiment, elemental property statistics are used as the basic features which are obtained by computing the mean, mean absolute deviation, range, mode, minimum, and maximum of 22 different elemental properties.

Random forest is an ensemble method that improves the model performance by constructing several weak algorithms (decision trees). \hl{In this work, we choose ‘entropy’ as our criterion. The two important hyper-parameters, 
the number of trees and max features, are set to be 100 and 80 respectively. The max depth is None. The min samples leaf and min samples split are sat as 1 and 2. This algorithm was implemented by the Scikit-Learn library in Python 3.6}

% It builds several estimators independently and each estimator gets the probability of possible output labels. Then the average of the predicted probabilities of all estimators is calculated as outputs. Labels with the highest average probability are used as the output results.

The Magpie descriptors based Deep Neural Networks (DNN) is also used in our work. \hl{The structure of our DNN model, shown in Fig. 2, is composed of 7 fully connected layers, and the numbers of the hidden nodes are 230, 178, 280, 244, 181, 192 respectively. Relu is used as the action function for those layers. And after each layer except the last one, two strategies, Dropout and BatchNorm, are used to prevent overfitting. The loss function is set as the categorical cross entropy loss. 
The Adam optimizer is used in model training. The learning rate, epochs and batch size are set as 0.001, 2000 and 255 respectively. In order to prevent overfitting and improve the performance of the DNN, we use the early stopping strategy where the monitor is ‘loss’ and patience is 30. Our DNN model is implemented on TensorFlow2.4.}

  



%{\textbf{\color{blue}Steph, Please write how GATGNN was developed to predict $E_\mathrm{form}$.}}
\fi

\iffalse
\subsection{Catalogue of structural motifs based on coordination numbers}

\subsection{variations and patterns of motifs of C.N.=4,5,7}


\hl{The number of atoms in a building block has the greatest influence on its shape. The number of atoms in each building block ranges from 3 to 19. Therefore, we first divide the building block into 17 categories according to the number of atoms in the building block, and then cluster each category}

\lipsum[2]

\subsection{variation and patterns of motifs of oxides}



\hl{what types of polyhedra for oxides}

show distribution figure (histogram)



\subsection{variation and patterns of motifs of lithium compounds}

\hl{what are the polyhedra around li-atoms}

\begin{equation}
    \mathrm{Accuracy} = \frac{1}{N} \sum^{N}_{i=1}(V^{\mathrm{DFT}}_i - V^{\mathrm{ML}}_i)
\end{equation}

\begin{equation}
    \mathrm{Roc} = 1- \frac{\sum^{N}_{i=1}(V^{\mathrm{DFT}}_i - V^{\mathrm{ML}}_i)^2}{\sum^{N}_{i=1}(V^{\mathrm{DFT}}_i - \overline{V})^2}
\end{equation}

Here, MAE is the mean absolute error and $\mathrm{R}^2$ is the coefficient of determination. $V^\mathrm{DFT}_i$ represents the voltage computed from DFT for $i^\mathrm{th}$ battery framework, and $V^\mathrm{ML}_i$ indicates the corresponding machine learning predicted voltage. $\overline{V}$  and $N$ are the number of data and the average voltage in the test set, respectively. In Fig.~\ref{fig:voltage}, the voltage predicted using machine learning models (ML-Voltage) vs the voltage calculated using DFT (DFT-Voltage) is shown for both reaction- and $E_\mathrm{form}$-based models. 

\textcolor{black}{Our method provides nearly 17 \% improvement when compared to previous approaches on the same data\cite{Rajendra1, Rajendra2}}. 

\fi
